Positional Identifiability from Pairwise Collision Data

We study the problem of recovering the relative positions of objects moving along the real line based only on pairwise collision data. While interaction-based sensing systems arise naturally in a variety of practical settings, a systematic theoretical understanding of positional identifiability from collision observations alone remains unexplored. Our contributions are three-fold. First, under the full observability model, in which both the set of collisions and their temporal ordering are known, we show that the relative positions of all objects can be uniquely recovered if and only if the collision history, represented as a graph, is connected. Second, we show that under partial observability, where only colliding pairs are observed without timing information, the problem is related to \emph{function graphs} and introduce a canonical layer decomposition in which each layer corresponds to a maximal clique; the contraction graph induced by this decomposition is an interval graph, and we provide efficient algorithms to recover it. Third, under incomplete observations where even some pairwise collision observations may be missing, we formulate the problem as a graph completion problem and establish its NP-hardness via a $4$-approximation relationship with the graph bandwidth problem.

==> abstract.tex <==

\begin{abstract}
We study the problem of recovering the relative positions of 
objects moving along a real line from pairwise collision data 
alone. While interaction-based sensing systems arise naturally 
in a variety of practical settings, a systematic theoretical 
understanding of positional identifiability from collision 
observations across different levels of observability remains 
lacking. Our contributions are three-fold. First, under full 
observability, where both the set of collisions and their 
temporal ordering are known, we show that the relative 
positions of all objects can be uniquely recovered if and only 
if the collision history is connected. Second, under partial 
observability, where only the set of colliding pairs is 
observed without timing information, we connect the problem 
to the theory of function graphs and introduce a canonical 
layer decomposition in which each layer corresponds to a 
maximal clique; the contraction graph induced by this 
decomposition is an interval graph, and we provide efficient 
algorithms to recover it. Third, under incomplete observations, 
where some collisions may be missing, we formulate a graph 
completion problem and establish its NP-hardness via a 
4-approximation relationship with the graph bandwidth problem.
\end{abstract}

==> old_stuff/old_3.7.tex <==
\subsection{Fixed-order set without time label}

In practice, we might not see the ordering of collisions. Therefore, in this section, we study the case with observation $\hg = (\mV,\E)$. being a simple graph with unordered edges.

We aim to recover the fixed-ordering (up to flip) for any fixed-order set $\foS\subset\mV$.
Note that it suffices to focus on those maximal fixed-order sets, since others can be deduced from them.
Let $\foS\subset\mV$ be a maximal fixed-order set and $\W\subset\mV$ be the set of neighbors of $\foS$. Then $\foS,\W$ partition $\mV$ since $\mv\notin\foS\bigcup\W$ implies $\foS\bigcup\{\mv\}$ is an independent set and therefore by Lemma~\ref{fxod_idps}, being a bigger fixed-order set.
For each $\w\in\W$, let $\foS_{\w}$ be the set of neighbors of $\w$ in $\foS$.
Let $\p=\mv_{1},\mv_{2},\hdots,\mv_{|\foS|}$ be the underlying fixed-ordering of $\foS$.

We have the following observations.
\begin{enumerate}
    \item Each $\foS_{\w}$ is an interval set, which means that the elements of $\foS_{\w}$ together are a substring on $\p$.
    \item For each $\w\w^{'}\in\E$, $\foS_{\w}\bigcup\foS_{\w^{'}}$ is also an interval set. Otherwise, there exists $\mv\in\foS\backslash\lp\foS_{\w}\bigcup\foS_{\w^{'}}\rp$ such that $\foS_{\w},\foS_{\w^{'}}$ is on a different side of $\mv$. But then one of $\w,\w^{'}$ should have a collision with $\mv$.
\end{enumerate}
Let $\clS$ be the collection of all these sets. Let $\p$ be a permutation of $n$ objects. We say $\clS$ admit $\p$ if all sets in $\clS$ are interval sets on $\p$. We are interested in all permutations that are admitted by $\clS$, since they are potential candidates for the underlying fixed-ordering.

\begin{lemma}
    $\clS$ admits a unique permutation (up to flip) iff the following conditions hold.
    \begin{enumerate}
        \item $\nexists\s_{1}\neq\s_{2}\in\foS$ with the same set of neighbors.
        \item $\nexists\foS^{'}\subset\foS$ with $1<|\foS^{'}|<|\foS|$ such that all $\cl\in\clS$ intersect with $\foS^{'}$ is a subset of $\foS^{'}$.
    \end{enumerate}
    Moreover, Algorithm~\ref{alg:dendongram} recovers the unique permutation.
\end{lemma}
\begin{IEEEproof}
    If $\clS$ violates condition 1, then $\exists \s_{1}\neq\s_{2}\in\foS$ such that for all $\cl\in\clS$, either $\{\s_{1},\s_{2}\}\subset\cl$ or $\{\s_{1},\s_{2}\}\bigcap\cl=\emptyset$.
    Let $\clS$ admit $\p$, then $\clS$ also admit $\p$ with $\s_{1},\s_{2}$ swap positions. Therefore, $\p$ is not unique. 

    Assuming condition 1 holds, then Algorithm~\ref{alg:dendongram} returns the unique permutation (up to flip) if condition 2 holds. Otherwise return all maximal sets $\foS^{'}\subset\foS$ that violate condition 2.
    For the first case, see that there cannot be $\s\in\p_{i}\backslash\cl$ standing between any $\s_{1},\s_{2}\in \lp\p_{i}\cap\cl\rp\bigcup\p_{i+1}$. Otherwise, $\cl$ is not an interval set. On the other hand, $\cl$ is an interval set for all permutations in the new description of each update.
    \begin{equation*}
        \p\leftarrow\p_{1},\hdots,\p_{i-1},\p_{i}\backslash\cl,\p_{i}\bigcap\cl,\p_{i+1},\hdots
    \end{equation*}
    Finally, after each update, $\cl\cap\p_{i}$ is either $\p_{i}$ or $\emptyset$ for all $i$. Combined with the fact that all future updates only change the permutation of elements within each $p_{i}$, we conclude that $\cl$ remains an interval set in all future updates. Consequently, all $\cl\in\clS$ are interval sets in the end, and therefore $\clS$ admits the returned permutation.

    For case 2, we show that all $|\p_{i}| > 1$ violate condition 2. For all $\cl\in\clS$, intersect with $\p_{i}$ implies $\cl\not\subset\p_{j},\forall j\neq i$. Therefore we have $\cl\subset\p_{i}$. Otherwise $\cl\not\subset\p_{j},\forall j$, then Algorithm~\ref{alg:dendongram} should not stop.
\end{IEEEproof}

\begin{algorithm}
  \caption{Recovering the fixed-ordering for any fixed-order set without time label} 
  \label{alg:dendongram}
  \begin{algorithmic}[1]
    \STATE \textbf{Input:} The clue set $\clS$. 
    %A maximal fixed-order set %$\foS\subset\mV$ with underlying fixed-ordering $\mv_{1},\hdots,\mv_{|\foS|}$.
    \STATE \textbf{Output:} Assuming condition 1 holds. If condition 2 also holds, then return the unique permutation (up to flip) admitted by $\clS$. Otherwise return all maximal sets that violate condition 2.
    \STATE \textbf{Initialization:} Pick two clues $\cl_{1}\neq\cl_{2}\in\clS$ with $\cl_{1}\cap\cl_{2}\neq\emptyset$. Let $\p=\p_{1},\p_{2},\p_{3}=\cl_{1}\backslash\cl_{2},\cl_{1}\cap\cl_{2},\cl_{2}\backslash\cl_{1}$.
    \STATE \textbf{Step 1: } Find a $\cl\in\clS$ such that $\cl\notin\p_{i},\forall i$.
    
    \STATE \textbf{Step 2: } $\forall \p_{i}$ with $\cl\cap\p_{i}\neq \p_{i},\emptyset$, exactly one of $\p_{i-1},\p_{i+1}$ intersect with $\cl$, say $\p_{i+1}$.
    \STATE $\p\leftarrow\p_{1},\hdots,\p_{i-1},\p_{i}\backslash\cl,\p_{i}\bigcap\cl,\p_{i+1},\hdots$.
    \STATE \textbf{Step 3: } $\clS\leftarrow\clS\backslash\cl$.
    \STATE goto \textbf{Step 1}
    \STATE \textbf{Step 4: } If all $|\p_{i}|=1$, return $\p$. Otherwise return all $|\p_{i}|>1$.

    
    
    %\STATE $UF(T,r)\leftarrow \max(UF(T_{1},r_{1}),UF(T_{2},r_{2})+1)$
    %\STATE \textbf{Return} $(\upd_{(T,r)}^{*},UF(T,r))$.
  \end{algorithmic}
\end{algorithm}




\subsection{Ongoing stuff}
In this section, we discuss ongoing stuff and generalizations.

\subsubsection{Distance comparison}
So far, we have only focused on recovering the fixed ordering of each fixed-order set. But we can deduce more from the history.
\begin{example}
There are four objects and two groups with ordering $\mv_{1},\mv_{2}$ and $\mv_{a},\mv_{b}$. At first $\mv_{a},\mv_{b}$ at far right and $\mv_{1},\mv_{2}$ at far left. Then $\mv_{a},\mv_{b}$ slide to left until passing $\mv_{1},\mv_{2}$ completly. By Lemma~\ref{fxod_idps} and Lemma~\ref{fxod_odering}, we can recover two groups and their fixed-ordering.

But we actually know more.
\begin{enumerate}
    \item If $\h = \mv_{2}\mv_{a},\mv_{1}\mv_{a},\mv_{2}\mv_{b},\mv_{1}\mv_{b}$, then we know $|\overline{\mv_{1}\mv_{2}}|<|\overline{\mv_{a}\mv_{b}}|$.
    \item If $\h = \mv_{2}\mv_{a},\mv_{2}\mv_{b},\mv_{1}\mv_{a},\mv_{1}\mv_{b}$, then we know $|\overline{\mv_{1}\mv_{2}}|>|\overline{\mv_{a}\mv_{b}}|$.
    \item If $\h = \mv_{2}\mv_{a},\{\mv_{2}\mv_{b},\mv_{1}\mv_{a}\},\mv_{1}\mv_{b}$, then we know $|\overline{\mv_{1}\mv_{2}}|=|\overline{\mv_{a}\mv_{b}}|$.
\end{enumerate}
\end{example}
In short, we can obtain some (but not all) distance comparisons ($> $, $ < $, $ =$) between pairs from different groups. This eventually gives us some partial ordering of distances between $\tbinom{|\G_{i}|}{2}$ pairs in each group $\G_{i}$·
So the question is: how much geometric understanding can we get for each group with this partial ordering information?

Moreover, in Corollary~\ref{fxod_coloring}, any coloring is a candidate for underlying groups. But these groups might not have coherent distance comparisons from history (Ex: $|\overline{\mv_{1}\mv_{2}}|>|\overline{\mv_{a}\mv_{b}}|$ at first but then $|\overline{\mv_{1}\mv_{2}}|<|\overline{\mv_{a}\mv_{b}}|$ later. In this case, we know at least one of $\{\mv_{1},\mv_{2}\},\{\mv_{a},\mv_{b}\}$ is not actually a group, even though they are all fixed-order sets. This cannot be deduced from Lemma~\ref{fxod_idps} and Lemma~\ref{fxod_odering}.) So, how much can we further narrow down possible groups after considering distance comparisons?

\subsubsection{High dimensional space}
We can extend the model into higher dimensions, say $2$. Everything is still the same except
Now objects are in $2$-dimensioanl space. 
Assuming we observe infinite long history, Then by analysis similar to Lemma~\ref{fxod_idps} and Lemma~\ref{fxod_odering}, we can 1) Get all candidate sets $\foS\subset\mV$ for groups 2) For each $\foS=\{\mv_{1},\mv_{2},\hdots\}$, we can get
the following information: Let $r>0$ be the distance such that two vertices visit each other if there are within distance $r$. Then for each pair $(\mv_{i},\mv_{j})$, we can get $d_{r}(\mv_{i},\mv_{j})$, which is defined as the minimum number of intermediate vertices a
witness have to visit between visit $\mv_{i}$ and visit $\mv_{j}$.
\begin{enumerate}
    \item When $d_{r}(\mv_{i},\mv_{j})=0$, it means there is a path from $\mv_{i}$ to $\mv_{j}$ such that there is no other vertices within distance $r$ from this path.
    \item When $d_{r}(\mv_{i},\mv_{j})=1$, it means there is a set of vertices $T\subset\mV$ such that $\bigcup_{u\in T}B_{r}(u)$ disect the whole space into two parts (inside and outside) with $\mv_{i},\mv_{j}$ lie in different parts.
    \item When $d_{r}(\mv_{i},\mv_{j})=2$, it means there are two layers...etc
\end{enumerate}
Then the question is: given $d_{r}(\mv_{i},\mv_{j}), \forall \mv_{i}\neq\mv_{j}\in\foS$, how much geometry information we can deduce from it? For example, what are those sets $T\subset \mV$ that dissect the whole space into two? And what is the "shape"of $T$? (Similar to the shape of a manifold)

Moreover, it is possible to define similarity between two different geometric distribution of objects by how long the history, and how much witness we need to separate their $d_{r}$ (for chosen $r$).
I don't know what application is suitable for this yet, but by changing $r$, this should have an interesting relation to persistent diagram mathematically.

\subsubsection{Missing history}
So far, we assume perfect history (observing every visit). But in practice, Visits are missing from time to time. 
A simple model for it is as follows.
As in Lemma~\ref{fxod_idps} and Lemma~\ref{fxod_odering}, let $\foS\subset\mV$ be a maximel fixed-order set, and $\W$ be the set of witness. We characterize imperfect history as follows: for each $\w\in\W$ with $\h_{\w}=\s_{1},\s_{2},\hdots$, there are at most $k$ missing between $\s_{i},\s_{i+1}$ for all $i$. So our previous result correspond to $k=0$, and the bigger the $k$ is, the more we missed.
We can still run Algorithm~\ref{alg:fixed-ordering}. But now each reported pair $(u,v)$ from the Algorithm only means they are within distance $k+1$ in the underlying
fixed-ordering instead of being neighbors.
The question is: what is the condition to recover the underlying fixed-ordering (or if it's impossible, how close we can approximate it in some sense? ) 
This should relate to the bandwidth problem a lot mathematically.


==> sec_future.tex <==
Many open problems in this new research area remain. Some of them are listed in what follows.
\begin{enumerate}
    \item \emph{Extend the results for the stretch and jump metric to apply to other types of graph-induced file models.} Despite sparse Hamiltonian and tree graphs being a good starting point for file modeling and analysis, it is clear that they represent an abstraction with practical limitations. For example, one can argue that instead of graphs, it is more appropriate to use unions of graphs, each of which models a different data file category. This setting can be analyzed in the same way as a single graph, but when the graphs are sparsely connected to form communities, the problem becomes significantly more challening.
    \item \emph{Extend the  characterization and conduct a more in-depth analysis of the redundancy-fragmentation trade-offs for different type of file graphs.} Since the trade-offs heavily depend on the properties of the file graphs, it would be relevant to first focus on bounds on the redundancy needed to achieve a certain fragmentation level, independent on the file graphs.
    \item \emph{Repeat and extend the results for other fragmentation metrics.} One can envision other metrics that are combinations of the stretch and jump metric (e.g., sum of stretches of individual jump fragments) or that take into account file integrity. In the latter case, not all permutations are allowed for the chunk store, but only those that respect \emph{batches} of unique chunks encountered in a file (i.e., breaking up bursts of unique chunks in files is not allowed).  
    \item \emph{Determine for what type of graphs adding coded redundant chunks outperforms simple chunk repetition.} Our examples show that the performance or repetition and linear coding may also depend on the allowed redundancy, which makes this problem challenging.
    \item \emph{Explore coding methods that involve more than $1$ redundant data chunk}. As deduplication necessitates significant reductions in the number of redundant chunks, to properly control fragmentation one may need to include more than one or two redundant or coded data chunks. We still have no general approaches for identifying which chunks to replicate or encode in this case. 
    \item \emph{Develop corresponding models for online setting.} The challenges associated with the online setting are that unique chunks already present in a file have to be stored in their natural order of appearance in the file. This implies that not all permutations of chunks are allowed for use in the chunk store.
    \item \emph{Simultaneously address fragmentation and robustness issues by using redundant or coded data chunks.} Although our initial analysis of fragmentation phenomena suggests that for file-graph models ``highly connected nodes'' are natural candidates for repetition, it is not clear if other, low-popularity chunks can also help in reducing fragmentation.
    \item \emph{Better analysis for bandwidth problem on Sparse Hamiltonian graph}.
    \item \emph{Characterization the middle part of the trade-off curves $S^{u}(G,m)$ and $J^{u}(G,m)$}.
    %\item repeat analyses for online deduplication (we exclusively worked with offline/postprocessing); in this case, chunks that come from the same file will necessarily have to be placed together, so we cannot arbitrary permute the content.
%    \item nonuniform chunk sizes
%    \item adding caching?
\end{enumerate}

\vspace{0.2in}
\textbf{Acknowledgement.} The authors are grateful to Hsing-Po Wang for suggesting to examine coding strategies other than pure repetition coding.

==> sec_jump.tex <==
We start this section with a discussion of the uncoded jump metric.  
%Therefore we can expect the trade-off curve for each $G$ as shown in Figure~\ref{fig:curve_detail_j}. 
We consider two extreme cases when there is no redundancy ($m=n$) and no fragmentation. In the later case, we seek the smallest $m$ such that $J^{u}_{t}(G,m)=1$. To position our ideas and approaches, we analyze trees in Section~\ref{sec_no_redundancy_j}, and then proceed to investigate fragmentation-free scenarios in Section~\ref{no_fragmentation_j}. Afterwards, we focus on the question of \emph{whether coding can improve the jump metric} in Section~\ref{SvCS_j}. The  cases where both redundancy and fragmentation are allowed are left for future analyses. 

\subsection{Deduplication Without Redundancy}\label{sec_no_redundancy_j}
As described in Section~\ref{sec:formulation}, to compute the uncoded jump metric $J^{u}_{t}(G,n)$ for the case when no redundancy is allowed, we proceed as follows. Given a graph $G=(V,E)$, we seek to find a length-$n$ chuck store $\cs$ that minimizes the number of runs of $1$s  in the binary vector $(\mathbbm{1}\{\cs_{1}\in p\},\mathbbm{1}\{\cs_{2}\in p\},\ldots,\mathbbm{1}\{\cs_{n}\in p\})$ for all paths $p\in P(G,\leq t)$. Clearly, $J^{u}_{t}(G,m)$ is a nonincreasing function of $m$. To the best of our knowledge, this problem was not previously considered in the  literature. 

We start with the case where $G=T$ is a tree and $t=n$, which means that the file system $P(T,\le n):=P(T)$ includes all self-avoiding paths in $T$. We provide an algorithm with time complexity $O(n)$ for finding an uncoded chunk store that offers a $4$-approximation for the jump metric $J^{u}_{n}(T,n)$. We conjecture that the problem of finding the exact jump metric $J^{u}_{n}(T,n)$ for trees is not NP-hard (unlike the problem of finding the stretch metric, which is NP-hard even for subclasses of trees such as caterpillars.)

%\vspace{-0.1in}
Figure~\ref{fig:tree1} depicts a \emph{caterpillar} graph. A caterpillar is a tree in which every branching node (i.e., a node of degree $>2$) lies on the same path called the body (marked in red). The remaining paths, which intersect with the body at only a branching node, are called hairs. The example in Figure~\ref{fig:tree1} has $12$ hairs. We can construct a linearization $s$ of the caterpillar examining the hairs in sequential order (say, from left to right), then writing out the nodes in each hair from the top (the node furthest away from the body) to the root of the hair, but excluding the branching node. Then, $\MinJ(s,p)\leq 3$ for all $p\in P(T)$ since each $p$ intersects at most two hairs and the body. This  implies that $J^{u}_{n}(T,n)\leq 3$. However, there are examples for which $J^{u}_{n}(T,n)<3$, as shown next.

\begin{figure}[H]
    \centering    \includegraphics[scale=0.24]{p8tree.pdf}
    \vspace{-0.25in}
    \caption{A caterpillar tree with $12$ hairs.} \label{fig:tree1}
    \vspace{-0.15in}
\end{figure}

The caterpillar in Figure~\ref{fig:tree2} has two hairs. A jump metric value of $J^{u}_{n}(T,n)=2$ can be achieved through the following linearization procedure. We first enumerate the left hair from the top to the root (the black node), the right hair from the root to the top, and finally, the path (body) of the caterpillar.

We start with some illustrative examples.

 The only possible paths corresponding to $3$ jumps are those starting from the left hair, going through the body, and then continuing on with the right hair. Their intersection with the two hairs corresponds to two paths starting from the black node and ending somewhere on the hair. These two paths end up being merged into a single run of $1$s in the linearization.   

To generalize these ideas for more general tree structures, we study another quantity termed the \emph{unidirectional path number}. For a rooted tree $(T,r)$ with $r\in V$, let $UP(T,r)\subset P(T)$ be the set of unidirectional paths on $T$. A path $p=v_{1},v_{2},\dots$ with $v_{i}\in V$ is called a unidirectional path if $v_{i}$ is a child of $v_{i+1}$ for all $i$. As an example, for a tree with three nodes, say $a,b,c$, where $b$ is the root node and $a$ and $c$ are its children, the path $p=abc$ is not unidirectional. The terminal nodes of the unidirectional path at the child and parent side are for simplicity called the bottom and the top of the path, respectively. %$MUP(T,r)\subset UP(T,r)$ is the set of maximal unidirectional paths (the bottom is a leaf and the top is the root).

\begin{figure}[H]
    \centering    \includegraphics[scale=0.24]{p9tree.pdf}
    \vspace{-0.2in}
    \caption{A caterpillar tree with $2$ hairs.}
    \vspace{-0.1in}
    \label{fig:tree2}
\end{figure}

An \emph{unidirectional path decomposition}, denoted by $\upd,$ is a set of disjoint paths $p\in UP(T,r)$ such that every node in $T$ is included in exactly one path. Let $UD(T,r)$ be the set of all unidirectional path decompositions. For any $\upd\in UD(T,r)$ and a file path $p\in UP(T,r)$, the \emph{unidirectional path number} $\F(\upd,p)$ is the number of paths in $\upd$ that intersect with $p$. The min-max unidirectional path number is defined as $$UF(T,r)=\min_{\upd\in UD(T,r)}\max_{p\in UP(T,r)}\F(\upd,p).$$
The following theorem shows that an optimal unidirectional path decomposition leads to a $4$-approximation for $J^{u}_{n}(T,n)$.
\begin{theorem}\label{main_theorem}
Let $T=(V,E)$ be a tree with jump metric $J^{u}_{n}(T,n)$, rooted at an arbitrary node $r\in V$. Let $\upd^{*}=\argmin_{\upd\in UD(T,r)}\max_{p\in UP(T,r)}\F(\upd,p)$ be an optimal unidirectional path decomposition, and let $\cs^{*}\in V^{n}$ be a linearization of the tree obtained by enumerating paths in $\upd^{*}$ in arbitrary order and direction (note that there are two possible directions to enumerate nodes on a path). Then, 
$$\max_{p\in P(T)}\MinJ(\cs^{*},p)\leq 4 J^{u}_{n}(T,n).$$ 
\end{theorem}
\begin{IEEEproof}
We have 
    \begin{align*}
        \max_{p\in P(T)}\MinJ(\cs^{*},p)&\overset{(a)}{\leq} \max_{p\in P(T)}\F(\upd^{*},p)\\
        &\overset{(b)}{\leq} 2 \max_{p\in UP(T,r)}\F(\upd^{*},p)\\
        &\overset{(c)}{=} 2 \min_{\upd\in UD(T,r)}\max_{p\in UP(T,r)}\F(\upd,p)\\
        %&\overset{(d)}{=} 2 \min_{d\in UD(T,r)}\max_{p\in MUP(T,r)}\F(d,p)\\
        &\overset{(d)}{\leq} 4 \min_{\cs\in V^{n}}\max_{p\in UP(T,r)}\MinJ(\cs,p)\\
        &\leq 4 \min_{\cs\in V^{n}}\max_{p\in P(T)}\MinJ(\cs,p)\\
        &=4 J^{u}_{n}(T,n),
    \end{align*}
    where 
    $(a)$ follows from the fact that $\cs^{*}\in V^{n}$ comprises paths in $\upd^{*}$. Since the intersection of two paths on a tree is still a path, for any file path $p\in P(T)$, the intersection of $p$ and each path in $\upd^{*}$ contributes at most one single run of $1$s on $\cs^{*}$ (two runs could merge into one if they are next to each other on $\cs^{*}$ like in the example of Figure~\ref{fig:tree2}). Consequently, the number of runs of $1$s on $\cs^{*}$ for each $p$ is $\MinJ(\cs^{*},p)\leq \F(\upd^{*},p)$; 
    $(b)$ follows from the fact that any path on $T$ can be split into two unidirectional paths. Let $p_{xy}\in P(T)$ with $x,y\in V$ be the path on $T$ from $x$ to $y$. Let $z\in V$ be the lowest common ancestor of $x,y$.  Then $p_{xy}=p_{xz}p_{zy}$ with $p_{xz}\in UP(T,r)$ and $p_{yz}\in UP(T,r)$. Since $\F(\upd^{*},p)$ is the number of paths in $\upd^{*}$ that intersect with $p$, $\F(\upd^{*},p_{x,y})=\F(\upd^{*},p_{x,z})+\F(\upd^{*},p_{z,y})-1\leq 2\max_{p\in UP(T,r)}\F(\upd^{*},p)$;
    $(c)$ follows from the fact that $\upd^{*}$ is optimal; %$(d)$ follows from the worst $\F(d,p)$ must from some maximal path. 
    $(d)$ follows from the following auxiliary  Theorem~\ref{main_tech}.
\end{IEEEproof} 
%$MUP(T)\subset UP(T)$ be the set of maximal unidirectional paths (start from a leaf to the root $r$). The minimum worst-case path number is defined as $$F_{r}(T)=\min_{d\in D_{r}(T)}\max_{p\in P_{r}(T)}\F(d,p).$$ Results in this section heavily rely on the following technical lemma.
\begin{theorem}\label{main_tech}
    For any rooted tree $(T,r)$, and linearization $\cs$ over $\mathbb{S}_n$, there exists a unidirectional path decomposition $\upd(\cs)\in UD(T,r)$ such that $\max_{p\in UP(T,r)}\F(\upd(\cs),p)\leq 2 \max_{p\in UP(T,r)}\MinJ(\cs,p)$.
\end{theorem}
\begin{IEEEproof}
Let $\cs$ be any chunk store of length $n$, and let $\cs_{i}$ denote the $i$-th entry of $\cs$. Furthermore, let $\cs_{i}^{j}$ stand for the substring of $\cs$ starting at  position $i$ and ending at $j$. Recall that $\MinJ(\cs,p)$ is the number of runs of $1$s in the binary vector $(\mathbbm{1}\{\cs_{1}\in p\},\mathbbm{1}\{\cs_{2}\in p\},\ldots,\mathbbm{1}\{\cs_{n}\in p\})$. 
%\iscomment{write $\cs'$ instead of $\cs^{'}$}
Similarly, for any subsequence $\cs'$ of $\cs$, $\MinJ(\cs',p)$ equals the number of runs of $1$s in $(\mathbbm{1}\{\cs'_{1}\in p\},\mathbbm{1}\{\cs'_{2}\in p\},\ldots,\mathbbm{1}\{\cs'_{|\cs'|}\in p\})$.

Let $1\leq i_{1}\leq n$ be the first position such that there does not exist a $p\in UP(T,r)$ that satisfies $\{\cs_{i}\}_{i=1}^{i_{1}}\subset p$; refer to this position as a break-point. Next, split $\cs=\cs_{1}^{i_{1}-1}\cs_{i_{1}}^{n}$ into two parts and repeat the procedure for $\cs_{i_{1}}^{n}$ to get a second break-point $i_{2}$, and continue until $\nb$ break-points $1<i_{1}<i_{2}<\ldots<i_{\nb}\leq n$ are obtained, so that $\cs=\cs_{1}^{i_{1}-1}\cs_{i_{1}}^{i_{2}-1}\ldots \cs_{i_{\nb-1}}^{i_{\nb}-1}\cs_{i_{\nb}}^{n}$ is partitioned into $\nb+1$ parts. Note that the segments $s_{i_j}^{i_{j+1}}$ cannot be covered by a single $p\in UP(T,r)$, although segments of the form $s_{i_j}^{i_{j+1}-1}$ can. 
%\iscomment{At this point, you should clarify to the reader what is the special property of this partition. Is it that each segment $s_{i_j}^{i_{j+1}}$ cannot be covered by a single $p$ (but each segment $s_{i_j}^{i_{j+1}-1}$ can)?}
%\iscomment{At this point, you should clarify to the reader what is the special property of this partition. Is it that each segment $s_{i_j}^{i_{j+1}}$ cannot be covered by a single $p$ (but each segment $s_{i_j}^{i_{j+1}-1}$ can)?}
Let $p_{0}\in UP(T,r)$, $p_{\nb}\in UP(T,r)$, and let the $p_{j}\in UP(T,r)$ be the shortest unidirectional paths that contain all vertices in
$\cs_{1}^{i_{1}-1},\cs_{i_{\nb}}^{n}$, and each $\cs_{i_{j}}^{i_{j+1}-1},$ respectively. Let $\upd(\cs):=\{p_{0},p_{1},\ldots\}$ be the collection of these paths.

We first observe  that for any break point $b$, $\MinJ(\cs,p)=\MinJ(\cs_{1}^{b},p)+\MinJ(\cs_{b}^{n},p)-\MinJ(\cs_{b},p)$. 
By repeatedly applying this equality to all breakpoints $\{i_{j}\}$ we arrive at
\begin{align*}
\MinJ(\cs,p)&=\MinJ(\cs_{1}^{i_{1}},p)+\sum_{j=1}^{\nb-1}\MinJ(\cs_{i_{j}}^{i_{j+1}},p)\\
    &+\MinJ(\cs_{i_{\nb}}^{n},p)-\sum_{j=1}^{\nb}\MinJ(\cs_{i_{j}},p)
\end{align*}
However, 
\begin{align*}
    2\sum_{j=1}^{\nb}\MinJ(\cs_{i_{j}},p)&\overset{(a)}{\leq}\MinJ(\cs_{1}^{i_{1}},p)+\MinJ(\cs_{i_{\nb}}^{n},p)\\
    &+\sum_{j=1}^{\nb-1}\lp\MinJ(\cs_{i_{j}},p)+\MinJ(\cs_{i_{j+1}},p)\rp\\
    &\overset{(b)}{\leq}\MinJ(\cs_{1}^{i_{1}},p)+\MinJ(\cs_{i_{\nb}}^{n},p)\\
    &+\sum_{j=1}^{\nb-1}\MinJ(\cs_{i_{j}}^{i_{j+1}},p),
\end{align*}
where 
$(a)$ follows from the fact that $\cs_{i_{1}},\cs_{i_{\nb}}$ are substrings of $\cs_{1}^{i_{1}},\cs_{i_{\nb}}^{n}$, respectively; $(b)$ follows from the fact that if $\MinJ(\cs_{i_{j}},p)=\MinJ(\cs_{i_{j+1}},p)=1$, then $\MinJ(\cs_{i_{j}}^{i_{j+1}},p)>1$.
Otherwise, $p$ would cover  $\cs_{i_{j}}^{i_{j+1}}$ and, by construction, no  $p\in UP(T,r)$ can cover $\cs_{i_{j}}^{i_{j+1}}$.
Consequently we have
\begin{align*}
    2&\MinJ(\cs,p)\\
    &\geq \MinJ(\cs_{1}^{i_{1}},p)+\sum_{j=1}^{\nb-1}\MinJ(\cs_{i_{j}}^{i_{j+1}},p)+\MinJ(\cs_{i_{\nb}}^{n},p)\\
    &\geq \mathbbm{1}\{\cs_{1}^{i_{1}-1}\cap p\}+\sum_{j=1}^{\nb-1}\mathbbm{1}\{\cs_{i_{j}}^{i_{j+1}-1}\cap p\}+\mathbbm{1}\{\cs_{i_{\nb}}^{n}\cap p\}.
\end{align*}
By the definition of the jump metric, 
\begin{align*}
    2&\max_{p\in UP(T,r)}\MinJ(\cs,p)\\
    &\geq \max_{p\in UP(T,r)}\mathbbm{1}\{\cs_{1}^{i_{1}-1}\cap p\}+\sum_{j=1}^{\nb-1}\mathbbm{1}\{\cs_{i_{j}}^{i_{j+1}-1}\cap p\}+\mathbbm{1}\{\cs_{i_{\nb}}^{n}\cap p\}\\
    &\overset{(a)}= \max_{p\in MP(T,r)}\mathbbm{1}\{\cs_{1}^{i_{1}-1}\cap p\}+\sum_{j=1}^{\nb-1}\mathbbm{1}\{\cs_{i_{j}}^{i_{j+1}-1}\cap p\}+\mathbbm{1}\{\cs_{i_{\nb}}^{n}\cap p\}\\
    &\overset{(b)}=\max_{p\in MP(T,r)}\mathbbm{1}\{p_{0}\cap p\}+\sum_{j=1}^{\nb-1}\mathbbm{1}\{(p_{j}\cap p)\}+\mathbbm{1}\{p_{\nb}\cap p\} \\
    &=\max_{p\in MP(T,r)} F(\mathcal{D}(s),p)=\max_{p\in UP(T,r)} F(\mathcal{D}(s),p)
\end{align*}
where $MP(T,r)\subset UP(T,r)$ is the set of maximal unidirectional paths, with the bottom corresponding to a leaf and the top to the root. Then, $(a)$ follows by the fact that $p$ should be a maximal unidirectional path; $(b)$ follows by that fact that if a maximal unidirectional path $p$ intersects with $p_{j}$, 
then $p$ must contain the node in $p_{j}$ that is ``closest'' to the root, which also belongs to $\cs_{i_{j}}^{i_{j+1}-1},$ since $p_{j}$ is the shortest unidirectional path that covers  $\cs_{i_{j}}^{i_{j+1}-1}$. 

The set of paths $\upd(\cs):=\{p_{0},p_{1},\ldots\}$ may not be a path decomposition yet since some of the paths may overlap. To resolve this issue, we repeatedly identify two intersecting paths $p_{i}$ and $p_{j}$. 
Let $c$ be the node at which they intersect that is closest to the root. Then, $c$ must be at the top of at least one of $p_{i}$ or $p_{j}$, say $p_{j}$. Otherwise, the parent of $c$ belongs to both $p_{i}$ and $p_{j}$, consequently being an intersecting node that is closer to the root than $c$.
Then, after removing $c$ from $p_{j}$, every node is still covered by $\upd(\cs)$, without an increase of $\F(\upd(\cs),p)$ for all $p\in UP(T)$. By repeating this procedure, $\upd(\cs)$ becomes a path decomposition with $\max_{p\in UP(T,r)}\F(\upd(\cs),p)\leq 2 \max_{p\in UP(T,r)}\MinJ(\cs,p)$. 
%\iscomment{from the previous equation, shouldn't the first max be $\max_{p\in MP(T,r)}$? but then this is not exactly the theorem statement?}
%\textcolor{red}{I increase a new line at the end of last chain of inequalities to make it into $\max_{p\in UP(T,r)}\F(\upd(\cs),p)$. }
%Subsection~\ref{mt_proof}.
\end{IEEEproof}
Theorem~\ref{main_theorem} reduces the problem of finding a $4$-approximation for the jump metric of trees to that of finding an optimal unidirectional path decomposition $\upd^{*}$. %Before we propose the algorithm, we further simplify the problem by the following observations. 
%\begin{enumerate}
    %\item Since no two paths in a unidirectional path decomposition can be merged into a longer one, the bottom of each path $p\in d^{*}$ must be a leaf. Otherwise, there must exist another $q\in d^{*}$ with the top being a child of the bottom of $p$. Then $pq$ is a longer unidirectional path. On the other hand, an unidirectional path cannot intersect with two leaves. Consequently, the number of paths in $d^{*}$ is exactly the number of leaves.
    %\item Since $\F(d^{*},p)$ is defined as the number of paths in $d^{*}$ that $p$ intersect with, $\max_{p\in UP(T)}\F(d^{*},p)=\max_{p\in MUP(T)}\F(d^{*},p)$. Therefore it suffices to consider the maximal file path (start from a leaf and end at root $r$).
%\end{enumerate} 
Algorithm~\ref{alg:path_number_rooted_tree} has complexity $O(n)$ and finds $\upd^*$ recursively. 

Let $\{r_{i}\}_{i=1}^{c}$ be the set of children of $r$, and let each $r_{i}$ be the root of a subtree denoted by $T_{i}$. Given a path decomposition $\upd\in UD(T,r)$, let $p=p'r\in \upd$ be the path in $\upd$ containing $r$. 
Then,  $(\upd\backslash \{p\})\cup \{p'\}$ is the union of path decompositions of the subtrees $(T_{i},r_{i})$. 
Hence, it suffices to first compute an optimal path decomposition for each of the subtrees, $\upd_{(T_{i},r_{i})}^{*}\in UD(T_{i},r_{i})$, evaluate the min-max unidirectional path number $UF(T_{i},r_{i})$ for each subtree $(T_{i},r_{i})$, and then extend one path among $\{p_{i}=p_{i}'r_{i}\in \upd_{(T_{i},r_{i})}^{*}\}$ to include $r$. Which path to extend can be determined as follows.  Without loss of generality, let $UF(T_{1},r_{1})\geq UF(T_{2},r_{2})\geq\ldots\geq UF(T_{c},r_{c})$. 
Suppose we chose to extend $p_{i}$. Then,  $\upd=\lp\lp\bigcup_{i=1}^{c}\upd_{(T_{i},r_{i})}^{*}\rp\backslash \{p_{i}\}\rp\bigcup \{p_{i}r\}$, and $\max_{p\in UP(T,r)}\F(\upd,p)=\max(UF(T_{1},r_{1})+1,UF(T_{2},r_{2})+1,\ldots,UF(T_{i},r_{i}),\ldots,UF(T_{c},r_{c})+1)$. Therefore the best choice for a path to be extended is $p_{1},$ and consequently,  $UF(T,r)=\max(UF(T_{1},r_{1}),UF(T_{2},r_{2})+1)$.   
%By the definition of path decomposition, our final path decomposition for $(T,r)$ must contain a path from some leaf to $r$. If the leaf is in $T_{1}$, then the worst case path number $F_{r}(T)=$
\begin{algorithm}
  \caption{Finding a min-max unidirectional path decomposition} 
  \label{alg:path_number_rooted_tree}
  \begin{algorithmic}[1]
    \STATE \textbf{Input:} $(T,r)$.
    \STATE \textbf{Output:} $(\upd_{(T,r)}^{*},UF(T,r))$.
    \STATE For each $(T_{i},r_{i})$, find $\lp \upd_{(T_{i},r_{i})}^{*},UF(T_{i},r_{i})\rp$. 
    \STATE $\upd_{(T,r)}^{*}\leftarrow \lp\bigcup_{i=1}^{c} \upd_{(T_{i},r_{i})}^{*} \backslash \{p_{1}\} \rp \bigcup \{p_{1}r\}$.\\ 
    Note that by definition, $p_i$ is the path in the decomposition $\upd_{(T_{i},r_{i})}^{*}$ that passes through node $r_i$. Since we found the decomposition, we know the path $p_i$.
    \STATE $UF(T,r)\leftarrow \max(UF(T_{1},r_{1}),UF(T_{2},r_{2})+1)$
    \STATE \textbf{Return} $(\upd_{(T,r)}^{*},UF(T,r))$.
  \end{algorithmic}
\end{algorithm}

\begin{figure}[H]
     \vspace{-0.1in}
        \centering
        \includegraphics[trim={0 3cm 0 1cm},clip,scale=0.26]{p8.pdf}
        \vspace{-0.1in}
    \caption{An example illustrating the process described in   Algorithm~\ref{alg:path_number_rooted_tree}. The black node is the chosen root node. The $16$ red nodes are leaves. The corresponding $16$ paths in the path decomposition are wide red lines.}
    %\label{psht}
\end{figure}

%Finally plug in Algorithm~\ref{alg:path_number_rooted_tree} into Algorithm~\ref{alg:path_number_tree}, we have an algorithm that can find an optimal path decomposition for tree $T$, and consequently a $\log(n)$ approximation of the jump metric $J^{u}_{n}(T,n)$ due to Theorem~\ref{thm:lognapproximation}. 



 

\subsection{Zero-Fragmentation Deduplication}\label{no_fragmentation_j}
By the definitions of the stretch and jump metrics, the smallest value of $m^{*}$ that allows one to achieve $J^{u}_{t}(G,m^{*})=1$ also forces $S^{u}_{t}(G,m^{*})=1,$ and vice versa. Therefore, the zero-fragmentation results for both metrics are the same.

\subsection{Coding Versus Repetition}\label{SvCS_j}
We address next the question of whether coding can help to reduce the jump metric. Specifically, we derive bounds on the difference $J^{u}_{t}(G,m)-J^{c}_{t}(G,m)$ and construct an example that shows that  $J^{u}_{t}(G,m)-J^{c}_{t}(G,m)>0$. The problem of finding the best coded chunk stores is difficult and left for future work. Also, we first consider chunk stores without redundancy ($m=n$) and then redirect our attention to stores with one redundant chunk ($m=n+1$).
\begin{theorem}\label{no_redundancy_j}
    We have $J^{u}_{t}(G,n)=J^{c}_{t}(G,n)$ for any file model \fm, which means that coding cannot improve the jump metric when no redundancy is allowed (i.e., when $m=n$). The result holds for both potential linear and nonlinear codes.
\end{theorem}
\begin{IEEEproof}
    The proof is similar to the proof of the results for the   stretch metric in  Theorem~\ref{no_redundancy} and is therefore omitted.
\end{IEEEproof}
When redundancy is allowed, Example~\ref{example1j} shows that coding can improve the jump metric even when only one redundant chunk ($m=n+1$) is inserted into the store.

\begin{example}\label{example1j}
Consider the file model $P(T,\leq n),$ with the generating graph $T$ depicted in Figure~\ref{fig:example1j}.
\begin{figure}[H]
 \vspace{-4.5mm}
    \centering
    \includegraphics[scale=0.24]{example1j.pdf}
    \caption{A tree $T=(V,E)$ with $8$ nodes.}\label{fig:example1j}
\end{figure}    

We start with the case of a chunk store with one redundant chunk ($m=n+1$). In this case, the uncoded jump metric satisfies $J^{u}_{n}(T,n+1)>2$. 
Suppose that there exists a length-$n+1$ chunk store $\cs$ with jump metric $\leq 2$. Since we can only duplicate one chunk, at least one of the sets of chunks from $\{\dc_{a},\dc_{1},\dc_{2},\dc_{3}\},\{\dc_{b},\dc_{4},\dc_{5},\dc_{6}\}$ (refer to the figures for chunk labels) is not duplicated in $\cs$, say $\{\dc_{a},\dc_{1},\dc_{2},\dc_{3}\}$. Let $\cs'$ denote the store $\cs$ after removing all replicas of $\dc_{b}$ (of which there may be at most two). Then, all $\{\dc_{i}\dc_{a}\dc_{j}\}_{i\neq j\in[3]}$ and $\{\dc_{i}\dc_{a}\dc_{b}\dc_{j}\}_{i\in[3],j\in[4:6]}$ must have a jump number $\leq 2$ with respect to $\cs$. This implies that all $\{\dc_{i}\dc_{a}\dc_{j}\}_{i\neq j\in[3]}$ and $\{\dc_{i}\dc_{a}\dc_{j}\}_{i\in[3],j\in[4:6]}$ must have a jump number $\leq 2$ with respect to $\cs'$ (since removing nodes does not lead to an increase in the jump metric). 
%\iscomment{but $\{\dc_{i}\dc_{a}\dc_{j}\}_{i\in[3],j\in[4:6]}$ are not paths on $T$?} 
There are two cases to consider for $\cs'$. The first case is that $\{\dc_{1},\dc_{2},\dc_{3}\}$ are all on the left of $\dc_{a}$ or all are on the right of $\dc_{a}$. The second case is that two of the three are on the left of $\dc_{a}$ and one at the right of $\dc_{a},$ or two of the three are on the right side of $\dc_{a}$ and one at the left side of $\dc_{a}$. We proceed with the first case, as the second case can be examined similarly.  Without loss of generality let $\cs'=\ldots\dc_{1}\ldots\dc_{2}\ldots\dc_{3}\ldots\dc_{a}\ldots$. If there exists any other chunk between $\dc_{3},\dc_{a}$, then $\dc_{1}\dc_{a}\dc_{3}$ has jump number $=3$ with respect to $\cs'$. 
Therefore $\cs'=\ldots\dc_{1}\ldots\dc_{2}\ldots\dc_{3}\dc_{a}\ldots$. Next, we show that all the elements in $\{\dc_4,\dc_5,\dc_6\}$ are adjacent to either $\dc_1$ or $\dc_a$. Suppose on the contrary, that one of $\{\dc_{4},\dc_{5},\dc_{6}\}$, say $\dc_{4}$, is not adjacent to $\dc_{1}$ or $\dc_{a}$ with respect to $\cs'$. Then $\dc_{1}\dc_{a}\dc_{4}$ has jump number equal to $3$ with respect to  $\cs'$. 
%\iscomment{but $\dc_{1}\dc_{a}\dc_{4}$ is not a path on $T$?}
Therefore,  without loss of generality, we can assume that $\cs'=\ldots\dc_{4}\dc_{1}\dc_{5}\ldots\dc_{2}\ldots\dc_{3}\dc_{a}\dc_{6}\ldots$. In this case, $\dc_{1}\dc_{a}\dc_{2}$ has jump number equal to $3$ with respect to  $\cs'$. Consequently,  $J^{u}_{n}(T,n+1)>2$.   
%By construction, $\dc_{a}$ has $3$ neighbors among $\{\dc_i\}_{i\in[6]}$. Therefore in any uncoded chunk store, at least one of them is not adjcient to $\dc_{a}$ on the chunk store, say $\dc_{1}$. 
%In addition, one of them must stand between another one and $\dc_{a}$. Consider $3$ different paths $\{\dc_{1}\dc_{a}\dc_{b}\dc_{i}\}_{i=4,5,6}$ on $T$. Notice  that all of them include $\dc_{1}$ and $\dc_{b}$. Since we have only one redundant chunk, at least one of them is not duplicated, say $\dc_{b}$. \textcolor{blue}{[previously we assume $x_a$ is not duplicated]} Then by the same reason, one of $\dc_{4},\dc_{5},\dc_{6}$ must stand between another one and $\dc_{b}$. Therefore there is always one path among three $\{\dc_{1}\dc_{a}\dc_{b}\dc_{i}\}_{i=4,5,6}$ that has jump metric $3$. 

On the other hand, the following coded chunk store has a jump number equal to $2$: 
\begin{equation*}
    \cs=\dc_{1}\dc_{a}\dc_{2}\dc_{3}(\dc_{a}\oplus \dc_{b})\dc_{4}\dc_{5}\dc_{b}\dc_{6}
\end{equation*}
Therefore, $J^{c}_{n}(T,n+1)\leq 2$.

To verify the claim, it suffices to check all paths of length $3$ and $4$ that can be recovered with $2$ jumps. The case of paths of length $3$ is easy to check. For paths of length $4$, we observe that we can
\begin{align*}
    \text{Recover }    &   \{\dc_{1},\dc_{2}\}\dc_{a}\dc_{b}\{\dc_{5},\dc_{6}\}\\
    ~&   \text{ from } \dc_{1}\dc_{a}\dc_{2}            ~&\text{ and } ~&\dc_{5}\dc_{b}\dc_{6}\\
    \text{Recover }    &   \dc_{3}\dc_{a}\dc_{b}\{\dc_{5},\dc_{6}\}\\
    ~&   \text{ from } \dc_{3}(\dc_{a}\oplus \dc_{b})   ~&\text{ and } ~&\dc_{5}\dc_{b}\dc_{6}\\
    \text{Recover }    &   \{\dc_{1},\dc_{2}\}\dc_{a}\dc_{b}\dc_{4}\\
    ~&   \text{ from } \dc_{1}\dc_{a}\dc_{2}            ~&\text{ and } ~&(\dc_{a}\oplus \dc_{b})\dc_{4}\\
    \text{Recover }    &   \dc_{3}\dc_{a}\dc_{b}\dc_{4}\\
    ~&   \text{ from } \dc_{a}              ~&\text{ and } ~&\dc_{3}(\dc_{a}\oplus \dc_{b})\dc_{4}
\end{align*}
The reduction of the jump metric achieved by coding is therefore 
\begin{equation*}
    J^{u}_{n}(T,n+1)-J^{c}_{n}(T,n+1)\geq 1.
\end{equation*}
\end{example}
The next result shows that for any file model and one redundant chunk, one can reduce the jump metric via coding by at most $2$. 
\begin{theorem}\label{coding_gain_j}
    We have $J^{u}_{t}(G,n+1)-J^{c}_{t}(G,n+1)\leq 2$ for any \fm, meaning that linear codes with one redundant chunk improve the uncoded jump metric by at most $2$.   
\end{theorem}
\begin{IEEEproof}
%We first show that all linear codes with one redundant chunk have at most one coded chunk as in  Example~\ref{example1j}.
Let $\cs=\cs_{1},\hdots,\cs_{n+1}$ be a length-$n+1$ coded chunk store in which each $\cs_{i}$ is a linear combination of a subset of user data chunks $\{\dc_{i}\}_{i=1}^{n}$. By the definition of the jump metric, it is required that for every file $p\in$ \fm\, comprising chunks in $X_{p}\subset \{\dc_{i}\}_{i=1}^{n}$, there exists a set of chunks $\cs_{X_{p}}\subset \cs_{[n+1]}$ of size $|\cs_{X_{p}}|=|X_{p}|$ such that $\cs_{X_{p}}$ can be used to recover $X_{p}$. Since all single chunks $\{\dc_{i}\}$ 
 belong to \fm, there are at least $n$ chunks in $\cs$ that are uncoded. Combining this claim with the fact that $m=n+1$, we conclude that there is at most one coded chunk in $\cs$.
 
Let $\cs^*$ be an optimal coded chunk store that achieves the jump metric $J^{c}_{t}(G,n+1)$. Let $\{\dc_{i_{1}},\dc_{i_{2}},\ldots\}\subset\{\dc_{i}\}_{i=1}^{n}$ and let, without loss of generality, $\cs^*_{j}=\sum_{\dc\in \{\dc_{i_{1}},\dc_{i_{2}},\ldots\}}\dc$ 
%\iscomment{This notation is strange. What is $\{a_i\}$? Is it a subset of $\{x_i\}_{i=1}^n$?}
be the only coded chunk in $\cs^*$. To recover each $X_{p}\subset\dc_{[n]}$, we can use the $n$ uncoded chunks in $\cs^*$ directly. If $\{\dc_{i_{1}},\dc_{i_{2}},\ldots\}\subset X_{p}$, then there exist $|\{\dc_{i_{1}},\dc_{i_{2}},\ldots\}|$ additional ways to recover $X_{p}$ by replacing one of the $\{\dc_{i_{1}},\dc_{i_{2}},\ldots\}$ in $\cs$ by $\cs_{j}$. Since we only remove one chunk and add another chunk, the increase of the jump metric is at most $2$. Therefore, we can create another uncoded chunk store $\cs'$ by removing $\cs_{j}$ from $\cs$. Then, all recovery sets for $\cs$ that do not use the coded chunk can also be used for $\cs'$, resulting in the same or smaller jump metric. Consequently $\cs'$ is an uncoded chunk store with jump metric $\leq J^{c}_{t}(G,n+1)+2$, which implies that $J^{u}_{t}(G,n+1)-J^{c}_{t}(G,n+1)\leq 2$.
\end{IEEEproof}
%\begin{corollary}
%    The proof above provides an intuition as of why coding helps. The set of original chunks $\{a_{i}\}$ can be understood as popular chunks shared by many files. We therefore apply coding on them so that $\{a_{i}\}$ can be reconstructed by $|\{a_{i}\}|+1$ different ways.
%\end{corollary}
%Finally, though jump metric for linear codes with one redundant chunk is only a base case, it might be more interesting when redundancy $\gg1$. 
Note that if we were to change the file model so that single-chunk files are prohibited, the arguments above for linear codes with one redundant chunk would no longer hold. %For example, an alternative file model can be an arbitrary collection of hyper edges (which are subsets of $\dc_{[n]}$).

==> sec_limits.tex <==
%\subsection{Fundamental limits for the non-adaptive case}
We first provide lower bounds for the smallest number of measurements needed for the $\mini{\Burstfx}$ and $\mini{\Burstbnd}$ settings. The proofs mostly use ideas from~\cite{colbourn1999}.
\begin{theorem}\label{LB_fix}\label{LB_variable} We have
    \begin{equation*}
        \begin{cases}
        \mini{\Burstfx}\geq \max\lp\log_{s+1}\lp n-\ell+1\rp,\lceil\frac{\ell}{2\threshold{s}}\rceil\rp,\\
        \mini{\Burstbnd}\geq \max\lp\log_{2}\lp n\rp,\lceil\frac{\ell}{s}\rceil\rp.
        \end{cases}   
    \end{equation*}
\end{theorem}

The proof technique used for $\mini{\Burstbnd}$ is similar to that for $\mini{\Burstfx}$; hence, we only provide the proof for $\mini{\Burstfx}$.   
We prove the first bound by establishing each of the bounds on the right-hand side separately and combining them via maximization. 
\begin{enumerate}
    \item The bound $\log_{s+1}\lp n-\ell+1\rp$ follows from a simple counting argument: there are a total of $n-\ell+1$ different head positions and a total of $s+1$ possible outcomes for each measurement.
    \item The bound $\lceil\frac{\ell}{2\threshold{s}}\rceil$: we show that even if we only require to discriminate among the first $\ell+1$ bursts (i.e., bursts $\burstwh{b}{i}$ with $0\leq i\leq\ell$), we still need $\lceil\frac{\ell}{2\threshold{s}}\rceil$ measurements. For any measurement $\bm{m}$, let $\bm{m}_{1}$ and $\bm{m}_{2}$ denote the first and second block of $\ell$ bits of $\bm{m}$. Only the last $\threshold{s}$ nonzero bits in $\bm{m}_{1}$ and the first $\threshold{s}$ nonzero bits in $\bm{m}_{2}$ are relevant. For simplicity, we only provide a proof for the $\bm{m}_{2}$ case. Let $\ell\leq i_{1}<i_{2}<\hdots<2\ell$ be the elements included in $\bm{m}_{2}$. Since $\length{b}=\ell$ and $\head{b}\leq\ell$, if $i_{j}$ is included in the burst $\burst{b}$ then $i_{1},\hdots,i_{j-1}$ must also be included. Therefore, if $j>\threshold{s}$, by observing that $\threshold{s}$ is the largest threshold, one can remove $i_{j}$ from $\bm{m}_{2}$ without changing the outcome. Hence one can only retain the first $\threshold{s}$ nonzero bits in $\bm{m}_{2}$ and still arrive at the same outcome. As a result, it suffices to only consider those $\bm{m}$ for which $\sum_{j=0}^{2\ell-1}\bm{m}(j)\leq 2\threshold{s}$. Let $\mb{M}^{h_{\mb{M}}\times 2\ell}$ be our measurement matrix restricted to the first $2\ell$ columns. Suppose that $h_{\mb{M}}<\frac{\ell}{2\threshold{s}}$; then $\sum_{i=0}^{h_{\mb{M}}-1}\sum_{j=0}^{2\ell-1} \mb{M}(i,j)\leq 2\threshold{s}h_{\mb{M}}<\ell$. This implies that there exists a $0\leq j<\ell$ such that $\mb{M}(*,j)=\mb{M}(*,j+\ell)=\bm{0}^{\height{\mb{M}}\times 1}$. Then $\thresholds\lp\mb{M}\burstwh{b}{i+1}\rp= \thresholds\lp\mb{M}\burstwh{b}{i}+\mb{M}(*,j+\ell)-\mb{M}(*,j)\rp=\thresholds\lp\mb{M}\burstwh{b}{i}\rp$. Therefore $\mini{\Burstfx}\geq \lceil\frac{\ell}{2\threshold{s}}\rceil$. 
\end{enumerate}









==> sec_practice.tex <==
%Data deduplication is a data reduction  technique employed in modern large-scale data storage systems that has the goal to increase storage efficiency by removing replicas of data stored by different users~\cite{comprehensive,kaur2018data,armknecht2015transparent,elrouayheb2016synchronization}.
Deduplication systems decompose files into chunks, then identify repeated and unique chunks using hash values, and then proceed to place the chunks into a chunk store. 

Hashing algorithms (such as SHA-1~\cite{penard2008secure} and MD5~\cite{kaliski1995message}) are used to produce hash values assigned to individual data chunks. For example, the MD5 hashing method is a \emph{message-digest one-way function} that takes as its input a message of arbitrary length and outputs a fixed-length hash as the message's signature; although originally designed for cryptographic protocols and message authentication in particular, it has found widespread applications in deduplication. Data chunks are termed \emph{unique} if they have not been stored before, and \emph{duplicates} if they are already present in the storage system. Both the unique and duplicate chunks are represented via hash values, and their presence in the cloud is detected through hashing rather than direct comparisons of their binary encodings.

Deduplication algorithms generally fall into two main categories: \emph{Inline} and \emph{post-processing} deduplication. 

Inline deduplication first deduplicates chunks in files arriving at the write path and then stores deduplicated data on the server. Inline deduplication requires few Input/Output operations but tends to highly scatter data chunks on the server and therefore leads to severe fragmentation (see~\cite{li2014efficient} for a more detailed discussion). To illustrate the process of inline deduplication, we denote the $j$-th %\iscomment{later, the notation $j$th is used, stick with one} 
data chunk by $\dc_{j}$ and provide an example of how to deduplicate three files in Figure~\ref{fig:inline}. When encountering the first file comprising two data chunks,  $(\dc_{4},\dc_{5})$, the server has no previously stored chunks, so both $\dc_{4}$ and $\dc_{5}$ are declared unique chunks and stored in consecutive linear order. Hence, the whole file (marked in red) is stored in one shot. When encountering the second file $(\dc_{2},\dc_{3},\dc_{4})$, only the chunks $(\dc_{2},\dc_{3})$ are unique (marked in red) and stored on the server. The process continues until the final chunk store content reduces to $(\dc_{4},\dc_{5},\dc_{2},\dc_{3},\dc_{1}).$ Since complete deduplication is performed, each chunk is stored only once, and the three files are represented by pointers to the store that include chunks of the files and their orders, e.g., $(1,2), (3,4,1), (5,3,1)$. Note that the pointers describe both the chunks as well as their orders within each individual file.

As opposed to inline deduplication, during post-processing deduplication one first stores all data chunks on the server, then deduplicates the content through an optimization process. An example of postprocessing deduplication is shown in Figure~\ref{fig:offline}, where as before one has to deduplicate the content of three files that arrived in some order. Instead of performing deduplication online, the post-processing deduplication algorithm considers the three files as a batch that is to be compacted jointly. In this particular example, the final chunk store content after postprocessing reduces to  $(\dc_{1},\dc_{2},\dc_{3},\dc_{4},\dc_{5}),$ and the three files are replaced by pointers as previously described. The file content is less fragmented in the post-processing chunk store than in the inline chunk store, which is easy to see in this case.
\begin{figure}[H]
 \vspace{-3mm}
    \centering
    \includegraphics[scale=0.27]{p0x_inline.pdf}
    \caption{Inline deduplication. Files arrive sequentially and are processed before being stored. Unique chunks from each file are marked in red, while the number of bars over a chunk symbol indicates the number of times it has been observed up to the given point in time.} \label{fig:inline}
\end{figure}
\begin{figure}[H]
 \vspace{-5mm}
    \centering
    \includegraphics[scale=0.27]{p0x_offline.pdf}
    \caption{Post-processing deduplication. Chunks are stored as soon as presented to the system (marked in red), and after all chunks are placed in the chunk store, duplicate chunks are removed and unique chunks reordered based on some optimization criteria.} \label{fig:offline}
\end{figure}
   
Although both methods of deduplication offer significant storage savings, it is clear from the above example that they introduce \emph{fragmentation}~\cite{li2014efficient,idedup,kesavan2020countering} and create problems with chunk \emph{robustness}~\cite{reliability,reliability2}. Data fragmentation refers to the already mentioned problem of storing information chunks of a file at multiple distal locations, which slows down data retrieval and potentially creates problems with accessing large volumes of secondary, unwanted interspersing data. For example, from the figure illustrating post-processing deduplication, one can observe that in order to restore the content of the third file, $(\dc_{1},\dc_{2},\dc_{4})$ one needs to read the first four chunks from the chunk store and then parse out the data chunk $\dc_{3}$.

Robustness, on the other hand, refers to the degree of tolerance of data loss in the file system when only one replica of each unique chunk is maintained. For example, from the figure illustrating post-processing deduplication, one can see that the data chunk $\dc_{4}$ is present in the files of all three users, but stored only once which may lead to a multi-client information loss in case the data chunk is compromised. Robustness problems are mitigated in practice by using specialized chunk placements and ``incomplete deduplication,'' where not all redundant chunks are removed but only a portion of them, as dictated by the popularity of the data~\cite{comprehensive}. In the context of the given example, this would suggest storing, say, one more copy of the chunk $\dc_{4}$.

The above discussion raises several natural questions. First, how does one have to place data chunks in a store to minimize some predefined fragmentation metric across all files? Second, can repeating a limited number of data chunks reduce the fragmentation metric for arbitrary or special collections of files? %A priori, it is unclear if redundancy actually reduces or increases fragmentation, since adding redundant chunks increases the number of chunks placed on the server that have to be potentially traversed during file reconstruction. 
Third, whenever redundancy helps, can \emph{coding across chunks} outperform simple \emph{repetitions}? Fourth, can carefully selected redundant chunks both reduce fragmentation and increase robustness simultaneously?

 \begin{figure}[H]
    \centering
    \includegraphics[scale=0.27]{p1x.pdf}
    \caption{An illustrative example of the trade-off between storage redundancy and fragmentation in deduplication systems. Blue and red lines correspond to the minimum number of fragments that need to be read to recover a file without accessing any chunks not in the file, and the minimum fragment length that covers all chunks of a file, respectively.}
    \label{fig:motivation}
\end{figure}
\begin{figure}[H]
 \vspace{-5mm}
    \centering
    \includegraphics[scale=0.27]{p2x.pdf}
    \caption{An illustrative example of the trade-offs among storage redundancy, fragmentation, and robustness in deduplication systems.} \label{fig:motivation2}
\end{figure}


To gain more insight into these questions, consider the examples in Figures~\ref{fig:motivation} and~\ref{fig:motivation2}. Figure~\ref{fig:motivation} provides an illustration of redundancy-fragmentation trade-offs. Suppose that we have to store three files with data chunks $(\dc_{4},\dc_{5})$, $(\dc_{2},\dc_{3},\dc_{4})$, and $(\dc_{1},\dc_{2},\dc_{4})$. If the three files are directly stored without deduplication, as shown in the figure, one needs to set aside space for a total of $8$ data chunks (bottom, right). To reduce the number of redundant data chunks stored, one might store each data chunk once (top, left), and as a result, the stored data chunk string is a permutation of $\dc_{1}$ to $\dc_{5}$. In this case, retrieving a file requires either a) accessing multiple segments of consecutive data chunks stored on the server to prevent reading extra data chunks that do not belong to the file, which is costly; or, b) reading a single or a small number of long data chunk fragments that include data chunks not originally in the file. As shown in Figure~\ref{fig:motivation}, different permutations of data chunks stored on the server result in different levels of fragmentation (a rigorous definition of fragmentation will be provided shortly). For example, when $(\dc_{1},\dc_{2},\dc_{3},\dc_{4},\dc_{5})$ is the chunk store string, the files $(\dc_{2},\dc_{3},\dc_{4})$ and $(\dc_{4},\dc_{5})$ can be read from one sequential fragment without including any unwanted chunks. However, when retrieving $(\dc_{1},\dc_{2},\dc_{4})$, one either needs two fragments to prevent reading unwanted  chunks $\dc_{4}$, or one longer fragment. 

\begin{figure}[H]
    \centering
    \includegraphics[scale=0.27]{p3x.pdf}
    \caption{An illustrative example of potential trade-off curves for storage redundancy versus fragmentation. The curves are file-graph specific, and shown for two different graphs using solid lines. The dashed lines correspond to the trade-off curves for the same file-graphs, but are meant to illustrate the potential gain achievable by allowing coding versus simple repetition redundancy. Note that these curves only serve as an illustration, and are not exact mathematical characterizations.} \label{fig:curve}
\end{figure}

Figure~\ref{fig:motivation2} is an illustration of the redundancy, fragmentation, and robustness trade-off paradigm. In this case, all three chunk stores ``lost'' their first chunk, and this compromises their performance differently. Chunk store $(\dc_{1},\dc_{2},\dc_{3},\dc_{4},\dc_{5})$ lost chunk $\dc_{1}$ and therefore lost one file $(\dc_{1},\dc_{2},\dc_{4})$. Chunk store $(\dc_{4},\dc_{5},\dc_{2},\dc_{3},\dc_{1})$ lost chunk $\dc_{4}$ and therefore lost all three files. Chunk store $(\dc_{4},\dc_{5},\dc_{2},\dc_{3},\dc_{4},\dc_{1},\dc_{2},\dc_{4})$ lost the first chunk $\dc_{4}$, but without compromising the integrity of the files. However, for the file $(\dc_{4},\dc_{5})$, the number of fragments that do not involve reading unwanted chunks increases from $1$ to $2$, and the read length for one consecutive fragment increases from $2$ to $4$. 

The goal of our work is to initiate the first mathematical study of redundancy and fragmentation trade-offs for post-processing deduplication (the study of redundancy, fragmentation, and robustness trade-offs for post-processing
settings will be addressed in a follow-up work). 
Specifically, we are interested in characterizing the trade-off curves for redundancy and fragmentation, for which potential examples are shown in~Figure~\ref{fig:curve}. The two solid lines are hypothetical trade-offs for two distinct file systems and simple repetition redundancy. Since coding in the form of redundant (non)linear combinations of chunks may lead to better results, two additional dashed lines are plotted to illustrate the potential gains. On each curve, two special points are highlighted in red, corresponding to the redundancy-free case, and blue, corresponding to the fragmentation-free case. To deduce relevant properties of these curves, we describe next the file and chunk models as well as the fragmentations metrics of interest.

%\begin{figure}[H]
%    \centering
%    \includegraphics[scale=0.27]{p3x.pdf}
%    \caption{An illustrative example of potential trade-off curves for storage redundancy versus fragmentation. The curves are file-graph specific \textcolor{red}{what is dashed, what is solid?}} \label{fig:curve}
%\end{figure}

==> sec_related.tex <==
%\subsection{Information Retrieval}
The work closest in terms of its approach to data storage is~\cite{coffey2000fundamental},  which established ultimate performance limits of information retrieval with and without data redundancy. One simple example to illustrate the problem is as follows. Assume that one wants to store a large image (i.e., a 2D grid of pixels) on a tape (i.e., a 1D storage media). The question of interest is how to store the pixels on the tape in a linear order to minimize the average access time of collections of pixels of walks/paths on the grid. Intuitively, the question asks to determine the effective reduction of 2D neighborhoods of pixels stored on a 1D tape. 

More precisely, assume that the image grid comprises $n\times n$ pixels. The system is initially in a state in which one of the pixels is displayed for the user, and the read–write head of the tape is located at a copy of the block stored on the tape.
The user generate a random sequence of requests for accessing pixels on the tape dictated by moves to one of the four neighboring blocks in the grid with uniform probability, and for each of the requests. After each request, the read head of the tape moves from its current location on the tape to the new position of the requested pixel, with access time measured by the moving distance.
The goal is to arrange all $n^2$ pixels on the tape in a manner that minimizes the average moving distance per time steps across all users generating random requests.

The problem therefore involves constructing a mapping between vertices of two graphs such that a given random walk on the first graph maps to an induced random walk on the second. The aim is to design the mapping so that the induced random walk on the second graph has as low an expected cost as possible. Specifically, let $V$ be the set of nodes of the $n \times n$ grid-graph, and let the graph be endowed with transition probabilities between pairs of adjacent states in $V$. The cost function of interest reads as 
\begin{equation*}
    E_C=\sum_{i,j\in V}p(i)\Pr(i,j)c(i,j), 
\end{equation*}
where $Pr(i,j)$ is the transition probability from state $i$ to state $j$ of the underlying irreducible Markov chain, and where $p(i)$ is the unique invariant probability distribution of the chain. The cost $c(i,j)$ is the distance between the vertices $i,j \in V$ on the tape (i.e., in the linear order).

When storing redundant pixels on the tape is allowed, the set of states of the storage system increases, and it is in general not entirely determined by the pixel currently being accessed. The system is now specified by an initial linear arrangement of pixels in the store, and a rule for deciding which state the system moves into given its current state and the next request. For example, with redundancy, we can store many copies of the same pixel on the tape. Then the rule must specify which of the several copies of a requested block is accessed. Nevertheless, we still operate under the assumption that the tape system states form an irreducible Markov chain. 
%The general problem with redundancy involves a mapping between two graphs with the number of vertices for that has the same number of vertices such that a given random walk on the first graph mapping to an induced random walk on the second. The problem is to design the mapping so that the induced random walk on the second graph has as low an expected cost as possible. Specifically, the expected cost is defined as
The expected cost in this case is defined as
\begin{equation*}
    E_C=\sum_{\ell\in L,j\in V}p(\ell)\Pr(\ell,j)c(\ell,j)
\end{equation*}
where $L$ is the redundant state space, and $Pr(\ell,j)$ are the transition probabilities of the Markov chain with redundant state space $L$. As before, $p(\ell)$ stands for the unique invariant probability distribution of the chain, while $c(\ell,j)$ denotes the cost of serving a request for block $j$ when the system is in state $\ell$, given the redundant  mapping of pixels to the tape.
Under this definition, unlike in our setting, it is not clear whether increasing redundancy always reduces the expected cost. For example, when we insert a new copy of a pixel on the tape, the cost of transitions between other states might increase since one needs to potentially cross one additional pixel on the tape. One of the main results in~\cite{coffey2000fundamental} shows
that when the file graph is a 2D $n \times n$ torus (i.e., wrapped grid) and the storage tape is a 1D loop (cycle), for the case of no redundancy ($m=n^{2}$), the optimal value of the objective scales as  $\Theta(n)$. However, with a small amount of redundancy (i.e., for $m=(1+\delta)n^{2}$ with a small constant $\delta$), the optimal value of the objective reduces to  $\Theta(1)$. The latter can be realized by repeatedly duplicating neighboring pixels across different granularities and then linearizing the 2D structure using a multi-layered raster scan, as illustrated in Figures~\ref{coffee1},~\ref{coffee2},~\ref{coffee3}, and~\ref{coffee4}.

\begin{figure}[H]
     \vspace{-0.1in}
        \centering
        \includegraphics[trim={0 3cm 0 4cm},clip,scale=0.26]{coffee1.pdf}
        \vspace{-0.1in}
    \caption{The first step is to recursively partition the torus into $g\times g$ subgrids until reaching an  individual pixel (in this example, via a $g=2\times 2$ partition).}
    \label{coffee1}
\end{figure}
\begin{figure}[H]
     \vspace{-0.1in}
        \centering
        \includegraphics[trim={0 3cm 0 4cm},clip,scale=0.26]{coffee2.pdf}
        \vspace{-0.1in}
    \caption{The second step is to create a redundant square grid in the first layer, by expanding the $g \times g$ grids into $(g+2)\times(g+2)$ grids, wrapped around at the boundaries according to the torus neighborhoods. For the example, the redundant subgrids are of size $4 \times 4$.}
    \label{coffee2}
\end{figure}
\begin{figure}[H]
     \vspace{-0.1in}
        \centering
        \includegraphics[trim={0 3cm 0 4cm},clip,scale=0.26]{coffee3.pdf}
        \vspace{-0.1in}
    \caption{In the next steps, the procedure described in the second step is repeated for the second, third etc layer, again using pixel subgrids of size $(g+2)\times(g+2)$.}
    \label{coffee3}
\end{figure}
\begin{figure}[H]
     \vspace{-0.1in}
        \centering
        \includegraphics[trim={0 3cm 0 4cm},clip,scale=0.26]{coffee4.pdf}
        \vspace{-0in}
    \caption{The final step is to linearize the redundant grid using a multi-layered (nested) raster scan.}
    \label{coffee4}
\end{figure}

==> sec_relatedwork.tex <==
The problem is closely related to the extensively studied `bandwidth problem' for graphs~\cite{diaz2002survey,petit2013addenda}:
%\begin{problem}
    Given a graph $G=(V,E)$, find a permutation $\sigma^{*}$ over $\mathbb{S}_n,$ the symmetric group of order $n$ that minimizes the worst-case edge stretch, $B(G):=\min_{\sigma}\max_{uv\in E}|\sigma(u)-\sigma(v)|.$
%\end{problem}
The graph bandwidth problem is NP-hard for general graphs. It is also NP-hard for trees with maximum degree $3$ and other subclasses of graphs~\cite{petit2013addenda}. The best known results for general graphs with efficient placement algorithms give an   approximation ratio of $O(\log^{3}(n)\sqrt{\log\log(n)})$ \cite{dunagan2001euclidean}. On the other hand, achieving an approximate within any constant $k\in N$ is NP-hard~\cite{unger1998complexity}. Still, for certain subclasses of graphs, more precise results can be derived. 

More specifically, the graph linearization and graph bandwidth problem are related as follows. Since the server chunk store  $s\in V^{n}$ is a permutation of $n$ chunks, $\forall w\in W(G,\leq t)$ we have $$\frac{\MinS(s,w)}{1+\ell(w)}\leq \frac{1+\sum_{i=1}^{\ell(w)}|s(w_{i})-s(w_{i+1})|}{1+\ell(w)}\leq \frac{1+\ell(w)B(G)}{1+\ell(w)}.$$ 
Furthermore, by the definition of the bandwidth, there exists $uv\in E$ such that $|s^{-1}(u)-s^{-1}(v)|\geq B(G)$. Together, these results imply that $\frac{B(G)}{2} \leq F_t(G,n) < B(G).$ In words, the bandwidth of a graph is an upper bound on the fragmentation level. Note that computing the bandwidth $B(G)$ for arbitrary graphs is computationally challenging, and existing general lower/upper bounds on $B(G)$ are mostly loose. This is why in the next section we turn our attention to a review of results from the graph bandwidth literature and subsequently focus on sparse Hamiltonian path graphs. The connection between the two problems for the case of a redundant chunk store is discussed in Section IV. Besides graph bandwidth, our problem is also related to a couple of graph optimization problems such as graph edgesum, profile width, pathwidth, cutwidth, cop and robber game, etc. Readers are referred to \cite{lai1999survey} for a comprehensive survey.
%\textcolor{red}{With the above definitions in place, we next turn our attention on providing bounds on the fragmentation level that do not rely on bandwidth results.} 
%For no redundancy, every vertex showed up exactly once (therefore $m=|V|$) in Problem~\ref{original_problem}, it's equivalent to finding the best permutation $\sigma$ over $V$ that minimizes the worst edge stretch.
%\begin{problem}[special case $m=|V|$]\label{bandwidth_problem}
%    Given a graph $G=(V,E)$, find $\sigma^{*}$ that achieve
%    \begin{equation*}
%        B(G):=\min_{\sigma}\max_{uv\in E}|\sigma(u)-\sigma(v)|
%    \end{equation*}
%\end{problem}    
%This problem is NP-hard for general graphs. Even remain NP-hard for trees with a maximum degree of $3$. 
%\iscomment{I think readers will find it a bit confusing that we introduce the fragmentation notion $F$, but then present most results in terms of $B(G)$. Would it be better to write $F_t(G,n)$ for the fragmentation level with files $W(G\leq t)$ and then use $F_2(G,n)$ instead of $B(G)$ (with the appropriate rescaling)?}

==> sec_summary.tex <==
Our results include both new bounds on the stretch metric $S^{u}_{t}(G,m)$, jump metric $J^{u}_{t}(G,m)$, and their coded counterparts $S^{c}_{t}(G,m),J^{c}_{t}(G,m),$ for the class of sparse Hamiltonian and tree-structured file-graphs, as well as algorithmic approaches for  constructing the resulting chunk stores. Most of the results hold for the special parameter values $t=2$ and $m=n+1$; these two limitations are a consequence of the difficulty of the underlying graph-theoretic problems and the requirement to keep the number of redundant data chunks as small as possible, respectively. Notable general results that pertain to arbitrary values of $t$ and graphs $G$ establish that when no redundancy is allowed (i.e., when $m=n$), coding cannot reduce neither fragmentation metric. When one redundant chunk is allowed (i.e., $m=n+1$), coding can reduce the stretch metric by a factor of at most two, and the jump metric by an additive term of at most two.
%By definitions, all of them are non-increasing function of $m$ that depends on the specific file model \fm. Our results are two parts. Part one is \emph{how much can coding help compared to repetition?} 
Illustration of the results are provided in Figures~\ref{fig:summary_S} and~\ref{fig:summary_J}.
\begin{figure}[H]
    \centering  
    \vspace{-0.1in}
    \includegraphics[scale=0.28]{psummary1.pdf}
    \caption{A possible pair of trade-off curves for the uncoded stretch metric $S^{u}_{t}(G,m)$ (solid line) and coded stretch metric $S^{c}_{t}(G,m)$ (dashed line) versus the chunk store size $m$. The two extreme ``corner points'' correspond to the case of no redundancy and no fragmentation.} \label{fig:summary_S}
\end{figure} 
\begin{figure}[H]
    \centering    \includegraphics[scale=0.28]{psummary2.pdf}
    \caption{Trade-off curves for the uncoded stretch metric $J^{u}_{t}(G,m)$ (solid line) and coded stretch metric $J^{c}_{t}(G,m)$ (dashed line) versus the chunk store size $m$. The two extreme ``corner points'' correspond to the case of no redundancy and no fragmentation.} \label{fig:summary_J}
\end{figure} 

In summary, for the stretch metric and all possible file models \fm, we have the following results.
\begin{enumerate}
    \item We prove in Theorem~\ref{no_redundancy} of Section~\ref{subsect:no_re} that $S^{u}_{t}(G,n)=S^{c}_{t}(G,n)$, which establishes that coding cannot help when no  redundant chunks are allowed (and therefore, the two red points in the previous figures coincide). Moreover, since $S^{u}_{t}(G,n)$ is closely related to the classical graph bandwidth which is difficult to find or bound for general graphs, we focus on bounding the stretch metric for sparse Hamiltonian graphs in Section~\ref{sec_no_redundancy}.
    \item We prove in Theorem~\ref{1bit_reduction} of Section~\ref{subsect:one_re} that $S^{u}_{t}(G,n+1)/S^{c}_{t}(G,n+1)\leq 2,$  which establishes that coding can at most halve the stretch metric with one redundant data chunk. We also present some explicit examples where coding reduces the stretch by a multiplicative factor of $2/3$.
    \item We prove in Theorem~\ref{no_fragmentation_coding} of Section~\ref{subsect:no_fra} that for $t=2$ coding cannot reduce fragmentation (i.e., the two blue points in the figures coincide). Moreover, Section~\ref{no_fragmentation}  establishes the connection between the problem in this setting and that of finding Eulerian paths in graphs. 
\end{enumerate}

For the jump metric and arbitrary file-graph models \fm, the results are similar to those presented for the stretch metric, as outlined below. 
\begin{enumerate}
    \item We prove in Theorem~\ref{no_redundancy_j} of Section~\ref{SvCS_j} that $J_{t}^u(G,n)=J_{t}^c(G,n)$, which establishes that coding cannot help when no  redundant chunks are allowed. Moreover, in Section~\ref{sec_no_redundancy_j} we establish bounds on $J_{t}(G,n)$ for trees $G$ and $t=n$ (i.e., for paths of all possible lengths in $G$), and the case when no redundant chunks are allowed. Our result is a $4$-approximation algorithm of complexity $O(n)$.
    \item In Section~\ref{SvCS_j}, Theorem~\ref{coding_gain}, we prove that for $m=n+1,$ $J^{u}_{t}(G,n+1)-J^{c}_{t}(G,n+1)\leq 2$, which implies that in this setting coding can reduce the jump metric by at most an  additive term equal to two. We also provide explicit examples of graphs for which coding can reduce the jump metric by one.
\end{enumerate}
